CAMEL: Co-Designing AI Models and Embedded DRAMs for Efficient On-Device Learning

On-device learning allows AI models to adapt to user data, thereby enhancing service quality on edge platforms. However, training AI on resource-limited devices poses significant challenges due to the demanding computing workload and the substantial memory consumption and data access required by deep neural networks (DNNs). To address these issues, we propose utilizing embedded dynamic random-access memory (eDRAM) as the primary storage medium for transient training data. In comparison to static random-access memory (SRAM), eDRAM provides higher storage density and lower leakage power, resulting in reduced access cost and power leakage. Nevertheless, to maintain the integrity of the stored data, periodic power-hungry refresh operations could potentially degrade system performance. To minimize the occurrence of expensive eDRAM refresh operations, it is beneficial to shorten the lifetime of stored data during the training process. To achieve this, we adopt the principles of algorithm and hardware co-design, introducing a family of reversible DNN architectures that effectively decrease data lifetime and storage costs throughout training. Additionally, we present a highly efficient on-device training engine named \textit{CAMEL}, which leverages eDRAM as the primary on-chip memory. This engine enables efficient on-device training with significantly reduced memory usage and off-chip DRAM traffic while maintaining superior training accuracy. We evaluate our CAMEL system on multiple DNNs with different datasets, demonstrating a $2.5\times$ speedup of the training process and $2.8\times$ training energy savings than the other baseline hardware platforms.

==> hpca-template-old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}


\begin{document}
\maketitle

%Enables the camera ready header and footer
\ifdefined\hpcacameraready 
  \thispagestyle{camerareadyfirstpage}
  \pagestyle{empty}
\else
  \thispagestyle{plain}
  \pagestyle{plain}
\fi

\newcommand{\hpcaheight}{0mm}
\ifdefined\eaopen
\renewcommand{\hpcaheight}{12mm}
\fi
  


==> tables/dudnn_arch.tex <==
\begin{table}
\centering
\caption{Position of Backbone DNN output. The names of DNNs indicate the number of layers in branch DNN and backbone DNN. For example, Branch-4 + ResNet-18 denotes a four-layer branch DNN with a ResNet-18 backbone.}
\begin{adjustbox}{width=0.8\columnwidth,center, cfbox=blue 1pt 1pt}
\begin{tabular}{|c|c|}  \hline
DNN &  Output layer indices  \\ \hline
Branch-4 + ResNet-18 &  4, 8, 12, 16\\
Branch-5 + ResNet-34 &  6, 12, 18, 24, 30\\
Branch-6 + ResNet-50 &  8, 16, 24, 32, 40, 48\\
Branch-6 + ViT-12 &  2, 4, 6, 8, 10, 12\\
Branch-6 + VGG-16 &  2, 4, 6, 8, 10, 12\\
Branch-8 + ViT-16 &  2, 4, 6, 8, 10, 12, 14, 16\\
Branch-12 + ResNet-50 & 4, 8, 12, 16, 20, 24, 28, 32, 36, 40, 44, 48 \\
Branch-12 + ViT-16 &  2, 4, 6, 8, 9, 10, 11, 12, 13, 14, 15, 16 \\\hline
\end{tabular}
\end{adjustbox}
\label{tab:dudnn-arch}
\end{table}

==> tables/pretrained-eval.tex <==
\begin{table}
\centering
\caption{\textcolor{blue}{The accuracies of the backbone DNN.}}
\begin{adjustbox}{width=\columnwidth,center, cfbox=blue 1pt 1pt}
\begin{tabular}{c|cccccc} \hline
DNNs       &  ResNet-18  & ResNet-34 & ResNet-50 & ViT-12 & ViT-16 & VGG-16 \\ \hline
CIFAR-10 &  71.77\%   &  73.08\%  &   74.22\%  &   72.96\%  &  73.08\%  &  73.17\%   \\\hline
Tiny-ImageNet  &  58.68\%   &  60.83\%  &   62.30\%  &  61.07\%   &  61.98\%  &  62.09\%   \\\hline
\end{tabular}
\end{adjustbox}
\label{tab:pretrained}
\end{table}

==> tables/retention-old.tex <==
\begin{table}
\centering
\caption{Data lifetime during the DuDNN training. "B", "R" and "V" denote Branch, ResNet and VGG, respectively. }
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{l|c|c|c|c} \hline
DNNs       &  B4+R18  & B5+R34 & B6+R50 & B6+ViT12 \\ \hline
lifetime   &    2.66$\mu$s  & 2.87$\mu$s   &  3.03$\mu$s  &   3.10$\mu$S \\ \hline
\#Refresh      &   0    &   0  &   0  &    0 \\\hline\hline
DNNs    & B6+V16 & B8+ViT16 & B12+R50 & B12+ViT16 \\\hline
lifetime &   3.86$\mu$s &  4.02$\mu$s    & 3.40$\mu$s  & 4.13$\mu$s   \\\hline
\#Refresh     & 1 & 1 & 1 & 1   \\\hline
\end{tabular}
\end{adjustbox}
\label{tab:datalife-time}
\end{table}

==> tables/text-eval.tex <==
\begin{table}
\centering
\caption{Training accuracies on text classification tasks.}
\begin{adjustbox}{width=0.65\columnwidth,center}
\begin{tabular}{l|c|c|c|c} \hline
Datasets &  DuDNN  & FI & CA & BrO \\ \hline
MRPC    &    0.822    &      0.830  &    0.676    &      0.404   \\
WNLI &    0.606   &      0.608 &   0.503   &      0.208  \\
RTE  &   0.648   &      0.655  &   0.611    &   0.341 \\\hline
\end{tabular}
\end{adjustbox}
\label{tab:text-result}
\end{table}
